Beam-Space MIMO Radar for Joint Communication and Sensing with OTFS Modulation

Motivated by automotive applications, we consider joint radar sensing and data communication for a system operating at millimeter wave (mmWave) frequency bands, where a Base Station (BS) is equipped with a co-located radar receiver and sends data using the Orthogonal Time Frequency Space (OTFS) modulation format. We consider two distinct modes of operation. In Discovery mode, a single common data stream is broadcast over a wide angular sector. The radar receiver must detect the presence of not yet acquired targets and perform coarse estimation of their parameters (angle of arrival, range, and velocity). In Tracking mode, the BS transmits multiple individual data streams to already acquired users via beamforming, while the radar receiver performs accurate estimation of the aforementioned parameters. Due to hardware complexity and power consumption constraints, we consider a hybrid digital-analog architecture where the number of RF chains and A/D converters is significantly smaller than the number of antenna array elements. In this case, a direct application of the conventional MIMO radar approach is not possible. Consequently, we advocate a beam-space approach where the vector observation at the radar receiver is obtained through a RF-domain beamforming matrix operating the dimensionality reduction from antennas to RF chains. Under this setup, we propose a likelihood function-based scheme to perform joint target detection and parameter estimation in Discovery, and high-resolution parameter estimation in Tracking mode, respectively. Our numerical results demonstrate that the proposed approach is able to reliably detect multiple targets while closely approaching the Cramer-Rao Lower Bound (CRLB) of the corresponding parameter estimation problem.

==> AlternativeBeamDesign.tex <==
\subsection{Beamforming matrices}\label{sec:bf_design}

The design of \ac{BF} matrix $\Fm$ at the radar \ac{Tx} depends on the operating phase. During the detection phase depicted in Fig. \ref{fig:Operational-Modes-a}, we choose $\Fm$ for a given angular sector such that both \ac{Tx} and \ac{Rx} are aligned towards the same wide angular sector. In this work we design the \ac{BF} matrix $\Fm$ based on %two different approaches, namely the Fourier based method following \cite[Section III.C]{friedlander2012transmit} and 
an optimization problem using the method of iterative thresholding.  
 
During the target tracking phase, we form multiple narrow beams corresponding to the estimated \ac{AoA} of the detected targets. This is illustrated with red and blue beams, corresponding to two different \ac{AoA}, in Fig.~\ref{fig:Operational-Modes-b}. Assuming that $P$ targets are detected and their respective AoA are estimated. Contrary to the transmit \ac{BF} matrix, the reduction matrix $\Um$ at the radar \ac{Rx} remains the same for both detection and tracking phases. Namely, by applying the Fourier based method following \cite[Section III.C]{friedlander2012transmit}, we set 
$\Um$,  where each column is given as 
\begin{align}
\uv_i = \left(\frac{\av(\theta_i)}{|\av(\theta_i)|}\right), \;\; i=1, \dots, \Nrf\,,
\end{align}
with a suitable normalization, where $\av(\theta_i)$ is defined in \eqref{eq:ULA}. This is illustrated in Fig.~\ref{fig:Rx-Beams}.  
This choice of an isotropic receive beam enables to obtain a multi-dimensional signal for \ac{AoA} estimation in both detection and tracking phases.


%\subsubsection{Fourier Beamforming}\label{Fourier_BF_Design}
%Following \cite[Section III.C]{friedlander2012transmit}, we construct $\Fm\in \CC^{\Na\times \Nrf}$ to cover a wide angular sector $[-\theta, \theta]$ as follows. 
%By representing this angular sector by a discrete set of $\Nrf$ angles, denoted by $\Theta=\left\{ \pm \left({\theta}/{(2\Nrf)} + k{\theta}/{\Nrf} \right)\right\}$, for $k=0,\dots,\Nrf/2-1$, we construct each column of $\Fm = [\fv_1, \dots, \fv_{\Nrf}]$ as 
%\begin{align}\label{eq:columnF}
%\fv_i = \frac{\av(\theta_i)}{|\av(\theta_i)|}, \;\; i=1, \dots, \Nrf\,,
%\end{align}
%with a suitable normalization, where $\av(\theta_i)$ is defined in \eqref{eq:ULA}. 

%During the target tracking phase, we form multiple narrow beams corresponding to the estimated \ac{AoA} of the detected targets. This is illustrated with red and blue beams, corresponding to two different \ac{AoA}, in Fig.~\ref{fig:Operational-Modes-b}. Assuming that $P$ targets are detected and their respective AoA are estimated, we construct $\Fm$ by replacing $\theta_i$ by $\hat{\phi}_p$  for the first $P$ columns in \eqref{eq:columnF} \cite[Section III.B]{friedlander2012transmit}.

%Contrary to the transmit beamforming matrix, the reduction matrix $\Um$ at the radar \ac{Rx} remains the same for both detection and tracking phases. Namely, we set 
%$\Um = \Fm^\H$,  where each column is given in \eqref{eq:columnF}. This is illustrated in Fig.~\ref{fig:Rx-Beams}.  
%This choice of an isotropic receive beam enables to obtain a multi-dimensional signal for \ac{AoA} estimation in both detection and tracking phases. 

%\subsubsection{Custom Designed Beampatterns}
In order to overcome the limitations of the simple and low complexity Fourier \ac{BF}, such as the definition of the main lobe shape and the inability to control the side lobe levels, for the construction of the \ac{BF} matrix $\Fm$, in this work we define an optimized pattern for each system operating phase. 

To obtain beam pattern sampled on $G$ grid points, the array factor matrix $\Am$ with dimensions $N\times G$ is defined as
\begin{align}\label{eq : ArrayFactor}
&\Am(\theta)=[ \av^{T}(\theta_1),... , \av^{T}(\theta_G)]\,,
\end{align}
where 
\begin{align}
&\theta_{g}\in{-\frac{\pi}{2}+\frac{\pi}{G}(g-1)},\quad g\in{1,..,G}\,,
\end{align}    
and the array manifold $\av$ of a generic $N$ element array is defined 
\begin{equation}\label{eq:strvec}
\av(\theta)=[ e^{j\frac{2\pi}{\lambda}d_{1}sin(\theta)},... , e^{j\frac{2\pi}{\lambda}d_{i}sin(\theta)}],\quad i\in \{1,...,N\}\,,
\end{equation} 
where $d_{i}$ is the position of the $i${-th} antenna element, which in the \ac{ULA} case, is an integer multiple of $\lambda/2$. The beam pattern radiated by the array at each sampling point of the grid can be calculated as the inner product of a weight (or excitation) vector $\omegav$ and the corresponding column of $\Am$. To this end, a desired beam pattern $b_{obj}(\theta)$ can be obtained by designing $\omegav$ such that
\begin{align}
%&\mathcal{B}(\theta)=\vec{a}^{T}(\theta)\omegav, \qquad\ \ \forall \theta \in \{ \theta_1 ... \theta_G\}\\
b_{obj}(\theta)=\av^{T}(\theta)\omegav, \qquad\ \ \forall \theta \in \{ \theta_1 ... \theta_G\}\,,
\end{align} 
where $\omegav = \left[{\omega_1,...,\omega_N}\right] $ is a weight vector defining the excitation value of each antenna element. 

The design problem of interest relies on finding a weight vector satisfying the demands on desired \ac{SLL} and \ac{FWHM} (i.e.,  pattern constraints). As a well known result, the \ac{FWHM} of an array is proportional to the electrical length or aperture of the array which is defined by the electrical distance between the first and last elements. Due to practical considerations, in this design problem we only consider element positions that are integer multiples of  $d_{0}=\lambda /2 $. Suppose we aim to steer the main beam of the \textit{normalized} radiation pattern in direction $\theta_{m}$,  with sidelobes below a predetermined bound $\rho_{K}$ over an angular region $\Theta_{K}$, then the problem is posed as
\begin{align}\label{eq:conditions}
  &\begin{cases}
   \av(\theta_m)^{T}\omegav=1 , & \theta = \theta_{m}\\
    \av(\theta)^{T}\omegav \leq \rho_{K} , & \forall \theta \in \Theta_{K}.
  \end{cases}
\end{align}

When steering the main beam direction toward wider angles, a beam squinting effect is observed such that the main lobe tends to broaden and grating lobes may also appear. Therefore, it is of interest to directly control the weight vector components corresponding to specific regions of the desired beam pattern corresponding to the reference mask. Considering the beam pattern design objectives of this work (see APPENDIX A), we formulate an optimization problem with the sparsity (i.e. $l_0$ norm) of the weight vector $\omegav$ as the optimization goal. In this regard we can define the constraint in \eqref{eq:conditions} as the main objective with the sparsity term as the \textit{regularizer} term. Given the non-convexity of the $l_0$ norm problem, finding the solution requires an intractable combinatorial search. Therefore, an alternative regularization method that has attracted considerable attention in the sparse signal processing and optimization literature is the $l_1$ -regularization, which aims to find the solution of
\begin{equation}\label{eq : l1_min_beck}
\underset{\xv}{\text{min}} \quad\left\{ F(\xv)\equiv\Vert \matr{\Xi}\xv-\bv\Vert^{2}_{2}+ \lambda\Vert \xv\Vert_1 \right\}\,,
\end{equation}  
where $\xv$ and $\matr{\Xi}$ are generic notations. 

Furthermore, a modification can be made to the $l_2$-norm least squares term in \eqref{eq : l1_min_beck}, treated as weighted least squares, such that the assignment of larger values to the components linked to certain sampling points forces the constraints on those regions (i.e., a smaller error for those directions).

By formulating the optimization problem \ref{eq : l1_min_beck} as below, we can find the minimizer of this  problem as derived in \cite{Beck_bf} 
\begin{align}\label{ist_def}
&\underset{\omegav}{\text{minimize}} \quad\Vert\omegav\Vert _{1}+ \gamma\Vert \Am\omegav-\bv_{obj}\Vert^2 _{2}\\
&\omegav^{(i+1)} = \underset{\omega}{\text{arg min}} \quad\Vert\omegav\Vert _{1} + \tau\gamma\Vert \omegav-(\omegav^{(i)}-\frac{1}{\tau}\nabla f(\omegav^{(i)}))\Vert^2_2
\end{align}  
This formulation is particularly suited to our design problem since adjusting $\gamma$ results in a trade-off between error and sparsity. In \cite{Beck_bf}, it is shown that smaller values of this parameter result in sparser solutions, however, since we are not interested in further sparsifying the derived array, it becomes possible to increase the value of $\gamma$ so that the derived pattern deviates from the objective mask with an smaller error. 
According to the description for the general step of ISTA  in Sec. 1 of\cite{Beck_bf}, 
we proceed further by taking a similar approach for the iteration steps of the fast iterative shrinkage thresholding algorithm described in section 4 of \cite{Beck_bf} and described in Algorithm \ref{alg:Fista}. 

\SetKwRepeat{Repeat}{Repeat}{\hspace{-0.3cm}Until}
\SetKwFor{For}{\hspace{-0.1cm}For}{do}{\hspace{-0.3cm}End}
\setlength{\algomargin}{0.1cm}
\begin{algorithm}
	\SetAlgoLined
	\justifying
	\noindent
	\noindent\textbf{Initialization:} Take $\yv^{1} = \omegav_0$, $t^{(1)}=1$ \;
	\noindent\For{$i\geq1$}
	{
		\begin{align}
		&\omegav^{(i)}=\Gamma_{\alpha} (\yv^{(i)}-\frac{1}{\tau}\nabla f(\yv^{(i)})) \\
		&t^{(i+1)}=\frac{1+\sqrt{1+4 (t^{(i)})^2}}{2}\\
		&\yv^{(i+1)}= \omegav^{(i)}+(\frac{ t^{(i)}-1}{t^{(i+1)}})(\omegav^{(i)}-\omegav^{(i-1)})
		\end{align}
		}
	\caption{\textit{FISTA}}
	\label{alg:Fista}
\end{algorithm}

%\begin{labeling}{}
%\item [Step 0]  
%\item [Step $i$ ] for $i\geq 1$ compute:
%\end{labeling}

%\begin{align}
%&\omegav^{(i)}=\Gamma_{\alpha} (\yv^{(i)}-\frac{1}{\tau}\nabla f(\yv^{(i)})) \\
%&\tv^{(i+1)}=\frac{1+\sqrt{1+4 (t^{(i)})^2}}{2}\\
%&\yv^{(i+1)}= \omegav^{(i)}+(\frac{ t^{(i)}-1}{t^{(i+1)}})(\omegav^{(i)}-\omegav^{(i-1)})\\
%\end{align} 

By defining the shrinkage operator $\Gamma_{\alpha}$ as in \cite{Beck_bf}
\begin{align}
\Gamma_{\alpha}(\omegav)_{i}= (\vert \omega _i \vert - \alpha)_{+} \text{sgn} (\omega_{i})
\end{align} 
we replace the  term $\Vert \Am\omegav-\bv_{obj}\Vert^2$ in \eqref{ist_def} with  $\Vert \Am\omegav-\bv_{obj}\Vert^2_{D}$  where  the weighted norm is introduced such that this weight controls the excitation values in each iteration. The weighted norm is defined as in section \ref{sec:Introduction} and the matrix $\matr{D}$ is a diagonal  
\begin{equation}
\mathbf{D}= 
 \begin{bmatrix}
    \,d_1 & 0&\cdots & 0\,  \\
    \,0&d_2 & \cdots & 0\,  \\
    \vdots  &  \vdots &\ddots & \vdots  \\
    \,0 & 0 &\cdots  & d_N\\
 \end{bmatrix}\,.
 \end{equation}

Then the gradient of the second optimization term denoted by $f(.)$ is given
\begin{equation}
\nabla f(\omegav) =\Am^{H}\Dm(\Am\omegav-\bv_{obj})\,.
\end{equation} 
To update the weights of $\Dm$ at every iteration we use the strategy proposed in \cite{Zhou_bf}, where the weight updates are non-decreasing. By defining the error from the desired beam pattern at a given angle on the grid and iteration $(i)$ as
\begin{equation}
r^{(i)}(\theta) = \vert \av(\theta)\omegav^{(i)} - \bv_{obj}(\theta) \vert\,,
\end{equation} 
The adjustment $s^{(i)}(\theta)$ of the weights is carried out as
\begin{equation}\label{eq:weight_update_synth}
  \begin{split}
  &\begin{cases}
   s^{(i)}(\theta) , & \theta \in \text{mainlobe region}\\
    \text{max}\left\{ 0,K_{p} r^{(i)}(\theta) \right\}, & \theta \in \text{sidelobe region}
  \end{cases}\,,
  \end{split}
\end{equation}
and
\begin{equation}\label{eq:weight_update_synth}
  \begin{split}
   s^{(i)}(\theta) =
  &\begin{cases}
   0, & \text{if} \quad r^{(i)}(\theta)<\epsilon \\
  K_{m} r^{(i)}(\theta) , & \text{otherwise}
  \end{cases}\,,
  \end{split}
\end{equation}
where $\epsilon$ is a design parameter such that a desired maximum error can be tolerated. $K_p$ and $K_m$ are gain factors of the weighing function and usually $K_m$ is specified to be much smaller than $K_p$ \cite{Zhou_bf}. These gain factors can be adjusted to reach a trade-off between sparsity, main-beam shape and side lobe attenuation levels in shaping the overall pattern. Numerical examples of beam patterns obtained with the aforementioned method are provided in APPENDIX A.   

==> PhysicalModel.tex <==
\begin{figure}
	\begin{subfigure}{.49\columnwidth}
		\centering
		\includegraphics[height=0.2\textheight]{BS_Broadcasting_H_Gtx_a.pdf}  
		\caption{Detection phase}
		\label{fig:Operational-Modes-a}
	\end{subfigure}
	\begin{subfigure}{.49\columnwidth}
		\centering
		\includegraphics[height=0.2\textheight]{BS_Broadcasting_H_Gtx_b.pdf}  
		\caption{Tracking phase}
		\label{fig:Operational-Modes-b}
	\end{subfigure}
	\caption{Two scenarios with two different Tx beam patterns. In (a), a Tx (a base station or a car) broadcasts a common message exploring a wide angular sector. In (b), we consider directional BF towards the detected targets.}
	\label{fig:Operational-Modes}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale=0.12]{Rx_Beams_Conf.pdf}
	\caption{Beam configuration at the radar Rx for the two scenarios depicted in Fig. \ref{fig:Operational-Modes}. $\Nrf$ beams cover a wide angular sector.}
	\label{fig:Rx-Beams}
\end{figure}


We consider joint radar detection and parameter estimation in a system operating over a channel bandwidth $B$ at the carrier frequency $f_c$.  We assume a \ac{Tx} equipped with a mono-static \ac{MIMO} radar with $\Na$ antennas and $\Nrf$ \ac{RF} chains, operating in full-duplex mode.\footnote{Full-duplex operations can be achieved with sufficient isolation between the transmitter and the (radar) detector and possibly interference analog pre-cancellation in order to prevent the (radar) detector saturation \cite{sabharwal2014band,wentworth2007applied,duarte2010fullduplexWireless}.}
The radar \ac{Rx} (which is located with the \ac{Tx}) processes the backscattered signal to identify the presence of targets within the beam, while estimating parameters of interest such as range, velocity, and \ac{AoA}. A point target model is taken into account, such that each target can be represented through its \ac{LoS} path only \cite{kumari2018ieee,nguyen2017delay,grossi2018opportunisticRadar}. By letting $\phi\in [-\frac{\pi}{2}, \frac{\pi}{2}]$ be the steering angle,  by considering an antenna array with $\lambda/2$ spacing ($\lambda$ is the wavelength), the \ac{Tx} and \ac{Rx} arrays are given by $\av(\phi)$ and $\bv(\phi)$ respectively, where $\av(\phi)=(a_1(\phi), \dots, a_{N_a}(\phi))^\T\in \CC^{N_a}$, denotes the uniform linear array response vector of the radar \ac{Rx} with 
\begin{align}\label{eq:ULA}
	a_n(\phi)&= e^{j(n-1)\pi \sin(\phi)},\;\; n=1,\dots, N_a,
\end{align}  
and $b_n(\phi)=a_n(\phi)$. Under the mono-static radar assumption, i.e., same angle $\phi$ at radar \ac{Tx} and \ac{Rx}, vectors $\av$ and $\bv$ result to be equal.
The channel is modeled as a $P$-tap time-frequency selective channel of dimension $\Na\times\Na$ given by \cite{vitetta2013wireless}
\begin{align}\label{eq:Channel}
	\Hm (t, \tau) =  \sum_{p=0}^{P-1} h_p \bv(\phi_p) \av^\H (\phi_p)\delta(\tau-\tau_p)  e^{j2\pi \nu_p t}\,,
\end{align}
where $P$ is the number of targets, $h_p$ is a complex channel gain including the pathloss, $\nu_p = \frac{2v_p f_c}{c}$ is the round-trip Doppler shift, $\tau_p=\frac{2r_p}{c}$ is the round-trip delay, and $\phi_p$ denotes the \ac{AoA}, each corresponding to the $p$-th target, respectively.
%
\subsection{OTFS Input Output Relation}\label{subsec:OTFS-Input-Output}
We consider \ac{OTFS} with $M$ subcarriers of bandwidth $\Delta f$ each, such that the total bandwidth is given by $B=M\Delta f$. We let $T$ denote the symbol time, yielding the \ac{OTFS} frame duration of $NT$, with $N$ number of symbols in time. We let $T\Delta f=1$, as typically considered in the \ac{OTFS} literature \cite{gaudio2019effectiveness,hadani2017orthogonal,raviteja2018interference}. 
In order to consider the aforementioned different operational modes, we let $\Ns$ denote the number of active \ac{RF} chains or data streams to be sent per time-frequency domain such that $\Ns=1$ corresponds to the multicasting of a single data stream and $\Ns\leq \Nrf$ corresponds to the broadcasting of individual data streams.
Following the standard derivation of the input-output relation of \ac{OTFS} (see, e.g., \cite{hadani2017orthogonal,gaudio2019effectiveness}), $\Ns$-dimensional data symbols $\left\{\xv_{k,l}\right\}$, for $k=0,\dots,N-1$, $l=0,\dots,M-1$, belonging to any constellation, are arranged in an $N\times M$ two-dimensional grid referred to as the Doppler-delay domain, i.e., $\Gamma=\left\{\left({k}/{NT},{l}/{M\Delta f}\right)\right\}$. 
% In order to send the block of symbols $\{x_{k,l}\}$, 
The \ac{Tx} first applies the \ac{ISFFT} to convert data symbols $\{\xv_{k,l}\}$ into a $\Ns\times1$ block $\{\Xm[n, m]\}$ in the time-frequency domain
\begin{equation}\label{eq:x-to-X}
\Xm[n,m]=\sum_{k=0}^{N-1}\sum_{l=0}^{M-1}\xv_{k,l}e^{j2\pi\left(\frac{nk}{N}-\frac{ml}{M}\right)}, 
\end{equation}
for $n = 0, \ldots, N-1$, $m = 0, \ldots, M-1$,  %and $i=1,\dots,\Nrf$.
satisfying the average power constraint $\EE[\Xm[n,m]^\H\Xm[n,m]]=\Pav/(NM \Ns) \Id_{\Ns}$, where $\Id_{\Na}$ denotes an identity matrix of dimension $\Ns$. 
% $\EE[|X_i[n ,m]|^2]\leq {\Pav}/{N_a}$, $\forall i$. 
% carries its own data stream, to be transmitted towards a given direction/target. The analysis considers the general case of $\Nrf$ different streams, while the generalization to a common message is straightforward.} 
%\footnote{Depending on the aforementioned operational modes, each \ac{RF} chain sends the same information, when the \ac{Tx} broadcasts a common message, or carries its own data stream, to be transmitted towards a given direction/target. The analysis considers the general case of $\Nrf$ different streams, while the generalization to a common message is straightforward.} 
%After assigning $\Ns$ streams to $\Nrf$ RF chains through a mapping matrix $\Vm\in \CC^{\Nrf \times \Ns}$ , 
Thus, the \ac{Tx} generates the $\Ns$-dimensional continuous-time signal
\begin{align}\label{eq:Tx-Signal-General}
\sv(t)  = \sum_{n=0}^{N-1} \sum_{m=0}^{M-1} \Xm[n, m] g_{\rm tx}(t-nT) e^{j 2\pi m \Delta f(t-nT)}.
\end{align}
Since the number of RF chains is typically much smaller than the number of antennas, different types of \ac{HDA} architectures between \ac{RF} chains and antennas have been considered in the literature (see e.g. \cite{song2019fully}). In this paper, we focus on the fully-connected \ac{HDA} scheme of \cite{song2019fully} while exploring and optimizing the analog \ac{BF} part. 
%{Given the fact that $\Nrf\ll\Na$, there is not a one-to-one mapping between \ac{RF} chains and antennas, which would require a fully digital \ac{BF} with $\Nrf=\Na$, %but some combining is necessary. To this end, two \ac{HDA} solutions are analyzed in \cite{song2019fully}. 
%, i.e., the fully-connected \ac{HDA}, in which each \ac{RF} is connected to all the antennas, and the partially-connected with one-stream-per-subarray \ac{HDA}, such that a different \ac{RF} chain belongs to a disjoint group of antennas. 
%Independently of the choice of an \ac{HDA} architecture, the key point is that the \ac{Rx} cannot access to each antenna element, but obtains only a projection of the received signal. This reflects in applying a \ac{BF} matrix, i.e., $\Fm$, at the \ac{Tx} side, which includes both baseband and \ac{RF} \ac{BF} (see \cite{song2019fully}), and a projection matrix $\Um$ at the \ac{Rx}. More details about the definition of such matrices can be found in \cite{song2019fully} and afterwords. In this paper the fully-connected \ac{HDA} scheme oh \cite{song2019fully} has been considered.
For any analog \ac{BF} architecture, the \ac{Tx} applies the \ac{BF} matrix denoted by $\Fm\in \CC^{\Na\times \Ns}$ that captures both baseband and 
\ac{RF} analog \ac{BF} (see \cite{friedlander2012transmit,fortunati2020mimoRadar}), while the \ac{Rx} sees the received signal of a reduced dimension through a projection matrix denoted by 
$\Um\in \CC^{\Nrf\times \Na}$. 
%By imposing $\trace(\Fm\Vm\Vm^\H\Fm^\H)=\Na$, the total power constraint $\Pav$ is satisfied. 
%the \ac{Rx} cannot access to each antenna element, but obtains only a projection of the received signal. This reflects in applying a \ac{BF} matrix, i.e., $\Fm$, at the %\ac{Tx} side, which includes both baseband and \ac{RF} \ac{BF} (see \cite{song2019fully}), and a projection matrix $\Um$ at the \ac{Rx}. 
%More details about the definition of such matrices can be found in \cite{song2019fully}. % and afterwords. 
% has been considered.

By transmitting the signal \eqref{eq:Tx-Signal-General} over the channel \eqref{eq:Channel}, the $\Nrf$-dimensional continuous-time received signal is given by 
\begin{align}\label{eq:Received-Signal-First}
	\rv(t) = \sum_{p=0}^{P-1} h_p {\Um} \bv(\phi_p) \av^\H(\phi_p)\Fm \sv(t-\tau_p) e^{j2\pi \nu_pt}\,.
\end{align}
%where we omitted the noise for the simplicity. Thus, note that the transmitted energy per symbol $\epsilon_{\rm s}$ satisfy the constraint 
%\begin{equation}
%	\epsilon_{\rm s}=\trace\left(\Fm\Vm\Id\frac{\Pav}{\Na}\Vm^\H\Fm^\H\right)=\frac{\Pav}{\Na}\trace\left(\Fm\Vm\Vm^\H\Fm^\H\right)=\Pav\,.
%\end{equation}
%$\Fm$ is a generic \ac{BF} matrix of dimension $\Na\times\Nrf$, with $\fv_i$ corresponding to the $i$-th column, or complex \ac{BF} vector, of dimension $\Na%\times1$, $\sv(t)$ collects the $\Nrf$ entries $s_i(t)$, {and $\Um$ is a $\Nrf\times\Na$ projection matrix}. 
%The choice of $\Um$ depends on the operational mode. Namely, during the detection/acquisition phase, we typically set $\Um=\Fm^\H$, such that both \ac{Tx} and \ac{Rx} are aligned towards the same wide angular sector. During the target tracking phase, while transmission is beamformed towards the targets (see Fig. \ref{fig:Operational-Modes} on the left side), reception is performed considering a wide angular sector (as in the first detection phase), such that a multi-dimensional signal is received, allowing \ac{AoA} estimation (as already explained in Section \ref{sec:Introduction}). In such a case, for instance, indicating with $\Fm_{(\bar{\theta}^\circ)}$ the \ac{BF} matrix covering an angular sector of $\bar{\theta}^\circ$ degrees, it results $\Um=\Fm^\H_{(\bar{\theta}^\circ)}$.


The output of the \ac{Rx} filter-bank adopting a generic receive shaping pulse $g_{\rm rx}(t)$ is given in \eqref{eq:y-received}, shown at the top of next page.
%, where $\Xm[n',m']$ is obtained by stacking the $\Nrf$ entries $X_i[n', m']$, i.e., $\Xm[n',m']=\left[X_1[n',m'],\dots,X_{\Nrf}[n',m']\right]^\T$.
\begin{figure*}
	\begin{align}\label{eq:y-received}
	\yv(t,f) &= \int  \rv(t')g^*_{\rm rx} (t'-t) e^{-j2\pi ft'} dt'= \int_{t'} g^*_{\rm rx} (t'-t) \sum_{p=0}^{P-1} h_p {\Um}\bv(\phi_p) \av^\H(\phi_p)\Fm\sv(t'-\tau_p) e^{j2\pi \nu_pt'} e^{-j2\pi ft'} dt'\nonumber\\
	&= 
	%\sum_{n'=0}^{N-1}\sum_{m'=0}^{M-1} \sum_{p=0}^{P-1} 
	\sum_{p,n',m'}h_p {\Um}\bv(\phi_p)\av^\H(\phi_p) \Fm \Vm \Xm[n', m']\int_{t'} g^*_{\rm rx} (t'-t)  g_{\rm tx}(t'-\tau_p-n'T) e^{j 2\pi m' \Delta f(t'-\tau_p-n'T)} e^{j2\pi (\nu_p-f) t'} dt'
	\end{align} 
\end{figure*}
By sampling at $t=nT$ and $f=m\Delta f$, we obtain
\begin{align}
\yv[n, m] &=\yv(t, f)|_{t=n T}^{f=m\Delta f}=\sum_{n'=0}^{N-1} \sum_{m'=0}^{M-1}\hv_{n,m}[n', m']\,,
\end{align}
where the time-frequency domain input-output relation $\hv_{n,m}[n', m']$ is given in \eqref{eq:time-frequency-h}, shown at the top of next page.
\begin{figure*}
	\vspace{-0.5cm}
	\begin{align}\label{eq:time-frequency-h}
	\hv_{n,m}[n', m']= \sum_{p=0}^{P-1} h'_p {\Um}\bv(\phi_p) \av^\H(\phi_p)\Fm  \Vm \Xm[n', m']C_{g_{\rm tx},g_{\rm rx}}((n-n')T -\tau_p, (m-m') \Delta f-\nu_p) e^{j 2\pi n' T \nu_p} e^{-j2\pi m \Delta f  \tau_p}
	\end{align}
\end{figure*}
Notice that we defined the cross ambiguity function $C_{u, v}(\tau, \nu) \eqdef \int_{-\infty}^{\infty} u(s) v^*(s-\tau) e^{-j 2\pi \nu s} ds$ as in \cite{matz2013time}, let $h'_p = h_p e^{j 2\pi \nu_p \tau_p}$, and imposed the term $e^{-j2\pi mn'\Delta f T}=1$, $\forall n',m$, under the hypothesis $T\Delta f=1$.
Since each $X_i[n, m]$ is generated via \ac{ISFFT}, the received signal in the delay-Doppler domain is obtained by the application of the \ac{SFFT}
\begin{align}
\yv[k,l]=\sum_{n,m}\frac{\yv[n,m]}{NM}e^{j2\pi\left(\frac{ml}{M}-\frac{nk}{N}\right)}=\sum_{k', l'}\gv_{k,k'}\left[l,l'\right],
\end{align}
where the \ac{ISI} coefficient of the Doppler-delay pair $\left[k',l'\right]$ seen by sample $\left[k,l\right]$ is given by
\begin{equation}
\gv_{k,k'}\left[l,l'\right]=\sum_p h_p' {\Um}\bv(\phi_p)\av^\H(\phi_p)\Fm\Vm\xv_{k',l'}\Psi^p_{k, k'}[l,l']\,,
\end{equation}
with $\Psi^p_{k, k'}[ l, l']$ defined in \eqref{eq:Psi-Mat}, shown at the top of next page.
%, and $\xv_{k',l'}$ obtained by stacking the $\Nrf$ entries $x_{i,k',l'}$, i.e., $\xv_{k',l'}=\left[x_{1,k',l'},\dots,x_{\Nrf,k',l'}\right]^\T$.
\begin{figure*}
	\vspace{-0.5cm}
	\begin{align}\label{eq:Psi-Mat}
	\Psi^p_{k, k'}[ l, l'] =\!\!\! \sum_{n, n', m, m'}\!\!\! \frac{C_{g_{\rm rx}, g_{\rm tx}}((n-n')T -\tau_p, (m-m') \Delta f-\nu_p)}{NM}  e^{j 2\pi n' T \nu_p} e^{-j2\pi m \Delta f  \tau_p}e^{j 2\pi \left(\frac{n'k'}{N}- \frac{m'l'}{M}\right)}e^{-j 2\pi\left(\frac{nk}{N}-\frac{ml}{M}\right)}
	\end{align}
	\noindent\rule{\textwidth}{0.4pt}
\end{figure*}
A simplified version of $\Psi^p_{k, k'}[ l, l']$ obtained by approximating the cross ambiguity function can be found in \cite{gaudio2019effectiveness}.


==> SimulationResults.tex <==
\section{Numerical Results}\label{sec:Numerical-Results}
\renewcommand{\arraystretch}{1.3}
\begin{table}
	\caption{System parameters}
	\centering
	\begin{tabular}{|c|c|}
		\hline
		$N=6$ & $M=512$ \\ \hline
		$f_c=24.25$ [GHz] & $B=150$ [MHz] \\ \hline
		$v_{\mathrm{res}}\simeq440$ [km/h] & $r_{\mathrm{res}}\simeq1$ [m]\\ \hline
		$v_{\mathrm{max}}=N\cdot v_{\mathrm{res}}$ & $r_{\mathrm{max}}=M\cdot r_{\mathrm{res}}$ \\ \hline
		$\Pav=40$ [mW] & $\sigma_{\mathrm{rcs}}=1$ [m$^2$] \\ \hline
		Noise Figure $=3$ [dB] & Noise PSD = $2\cdot10^{-21}$ [W/Hz] \\ \hline
	\end{tabular}
	\label{tab:System-Parameters}
\end{table}

The number of \ac{RF} chains $\Nrf=8$ is set such that a single equipment is able to jointly track and communicate to $\Nrf$ separately targets (or groups of targets), while $\Nrf\ll\Na$. Table \ref{tab:System-Parameters} provides the system parameters. 

In our simulations, we rely on the following assumptions:
\begin{itemize}
	\item Given the choice of a \ac{mmWave} communication, we assume \ac{LoS} between the \ac{Tx} and the \ac{Rx} (or radar target) \cite{kumari2018ieee,nguyen2017delay}. This is motivated by the fact that any possible scattering component different from the \ac{LoS} generally brings much lower power, given by additional reflections of the echo signal.
	\item Any backscattered power to the radar \ac{Rx} is considered as a possible target. The objective is to sense the surrounding environment, and the differentiation between active targets and obstacles is a post-processing decision. Clearly, in a second phase, communication is established only towards active target (there is no interest to send information to a tree). 
	\item We consider the complete blockage of the signal propagation to the first object hit. This assumption is completely fulfilled in \ac{mmWave} communication scenarios.\footnote{Note that the proposed algorithm could be able to correctly distinguish more targets sharing the same angular direction, if separated in at least one other domain (Doppler or delay) \cite{gaudio2020joint}.} 
\end{itemize}
Note that the aforementioned assumption are shared by many works in literature (see, e.g., \cite{grossi2018opportunisticRadar} and references therein).

% Following the approach of \cite{grossi2018opportunisticRadar}, which follows \cite{rappaport2012propagation,rappaport2015wideband}, 
The radar two-way \ac{PL} is defined as \cite[Chapter 2]{richards2014fundamentals}
\begin{equation}
	\mathrm{PL}=\frac{(4\pi)^3r^{4}}{\lambda^2}\,,
\end{equation}
% such that the standard \ac{PL} (see, e.g., \cite[Chapter 2]{richards2014fundamentals}) formula is obtained for $\eta=2$, while, at \ac{mmWave} at $f_c=24.25$ GHz \cite{braun2014ofdm,sturm2011waveform}, by properly taking into account additional gases absorption effects \cite{rappaport2012propagation}, a more precise formulation of the \ac{PL} requires $\eta=2.5$. 
and the definition of the radar \ac{SNR} becomes 
\begin{equation}
	\mathrm{SNR}=\frac{\lambda^2\sigma_{\mathrm{rcs}}G_\mathrm{Tx}G_\mathrm{Rx}}{\left(4\pi\right)^3r^4}\frac{\Pav}{\sigma_w^2}\,,
\end{equation}
where $\lambda=c/f_c$ is the wavelength, $c$ is the speed of light, $\sigma_{\mathrm{rcs}}$ is the radar cross-section of the target in $\mathrm{m}^2$, $G_\mathrm{Tx}$ and $G_\mathrm{Rx}$ are the antenna gains at the \ac{Tx} and \ac{Rx} respectively, $r$ is the distance between \ac{Tx} and \ac{Rx}, and $\sigma_w^2$ is the variance of the \ac{AWGN} noise with noise \ac{PSD} of $2\cdot10^{-21}$ [W/Hz]. We choose $\sigma_{\mathrm{rcs}}=1$ [m$^2$], while different choices can be found in literature \cite{suzuki2000measurement,kamel2017RCSmodeling}. Note that, while $G_\mathrm{Tx}$ can change with the operational mode, $G_\mathrm{Rx}$ is keep constant (within the angular sector of interest) in order to allow isotropic reception, as already explained. Information about antenna gains, beam patterns, two-way (\ac{Tx} and \ac{Rx}) beamwidth, and more antenna basics (also for mono-static radars) can be found, for instance, in \cite{visser2006array,friedlander2012transmit}.

While two distinct targets in the angle domain can be identified if the angular resolution meets some conditions (depending on the number of antennas, the angular distance between the two targets, and the antenna array properties) \cite{richards2014fundamentals}, a different analysis has to be done for Doppler and delay. In brief, given the parameters listed in Table \ref{tab:System-Parameters}, velocity and range resolutions are
\begin{equation}\label{eq:Radar-Resolution}
v_{\mathrm{res}}=\frac{Bc}{2NMf_c}\ \mathrm{[m/s]}\,,\:\:\:r_{\mathrm{res}}=\frac{c}{2B}\ \mathrm{[m]}\,.
\end{equation}
In order to get a reasonable range resolution, e.g., $<1$ [m], a large bandwidth has to be considered.\footnote{Note that a tradeoff appears. Larger bandwidths mean more precise resolution, but lower theoretical maximum range (with the same $N\times M$ grid). We remark that our algorithm is completely independent of these choices.} Since the velocity resolution is directly proportional to $B$, for a fixed $f_c$, the only way to obtain a lower values is to increase the block size $NM$, leading to a remarkable increase in computational complexity, which could be not affordable. For this reason, we set the system parameters by focusing on a reasonable range resolution (and theoretical maximum range) under a feasible computational complexity. Note that the maximum range could not be achieved if the \ac{PL} brigs the backscattered power below the noise floor. This in turn leads to an unavoidable very large velocity resolution. Note that, given the assumptions taken at the beginning of Section \ref{sec:Numerical-Results}, the problem of targets identifiability appears only in the angular domain, given the total blockage of the signal power within a given direction. However, this only happens at \ac{mmWave}, thus, range and velocity resolutions are reported here for completeness, since the proposed scheme could target lower frequencies, where the aforementioned assumption might not be satisfied. 

\begin{remark}
	The parameters estimation performance of the proposed \ac{ML}-based algorithm strictly depends on the dimension of the block of data sent, i.e., the product $N\cdot M$. Thus, the system parameters of Tab. \ref{tab:System-Parameters} can be easily tuned to achieve the desired levels of radar resolutions (modifying the bandwidth), acquisition time (based on the length of the \ac{OTFS} frame in time), maximum range, etc. Clearly, the \ac{CRLB} changes accordly. Moreover, note that this is also possible thanks to \ac{OTFS} modulation, which is not sensitive to Doppler and delay effects.   
\end{remark}

\begin{remark}
	Radar range and velocity resolutions indicates the minimum necessary targets spacing, in one of the two domain, such that both of them are distinguishable at the radar \ac{Rx}. This has not to be confused and it is not linked to the performance of our \ac{ML}-based detector, which is, indeed, a super-resolution method, able to produce radar parameters estimates with error remarkably lowers w.r.t. the aforementioned resolutions. Thus, there is a huge difference between targets identifiability and estimation performance.
\end{remark}

\begin{figure}
	\centering
	\includegraphics[scale=0.65]{./rangeVelocityAOA_BF_Range.pdf}
	\caption{\ac{Tx} broadcasting a common message. Single target at a different distance within the illuminated angular sector of specified coverage. RMSE performance with associated CRLB and detection performance. $N_a=128$.}
	\label{fig:Detection-Range-Na128}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale=0.65]{./rangeVelocityAOA_BF_2Targets.pdf}
	\caption{\ac{Tx} broadcasting a common message. Two target, one fixed at $10$ [m] and the other moving at a different distance (x-axis) within the illuminated $10^\circ$ angular sector. RMSE performance with associated CRLB. Detection performance. $N_a=128$.}
	\label{fig:Detection-Range-Na128-2Targets}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale=0.2]{./Fig2Ex.pdf}
	\caption{Example of scenario depicted in Fig. \ref{fig:Detection-Range-Na128-2Targets}. The moving target, in blue, changes its location. A masking effect is related to the fixed target.}
	\label{fig:Ex-Scenario-MovTarget}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale=0.63]{./rangeVelocityAOA_BF10_SNR.pdf}
	\caption{\ac{Tx} BF distinct beams towards three different targets. Reception is isotropic, thus AOA estimation is possible (See Fig. ... on the left). Different numbers of antennas. RMSE performance is calculated for one target, while the others are randomly placed and act as interference.}
	\label{fig:BF-Targets}
\end{figure}

\subsection{Simulation Results}
Fig. \ref{fig:Detection-Range-Na128} shows the acquisition performance in terms of \ac{Pd} for a \ac{Tx} broadcasting a common message (see Fig. \ref{fig:Operational-Modes}), while performing estimation of the parameters of interest of the (single) target within an angular sector of different width. First, note that, by considering an angular coverage of $10^\circ$ degrees, the maximum range to correctly identify a target, limited by the \ac{PL} and thus different from he theoretical limit indicated in Table \ref{tab:System-Parameters}, is about $110$ m. For any distance between \ac{Tx} and target, the estimation performance of radar parameters of interest (range, velocity, and \ac{AoA}) follows the corresponding \ac{CRLB}. More in details, note that at the limit range of $110$ m, the \ac{RMSE} for range, velocity, and angle are respectively, $\simeq4\cdot10^{-2}$ [m], $\simeq1.6\cdot10^{1}$ [m/s], $\simeq4\cdot10^{-2}$ [degree$^\circ$]. As expected, given the system parameters, the velocity \ac{RMSE} is quite poor, while the others estimation performance are satisfactory. However, a proper \ac{BF} design towards targets, in a successive tracking/communication phase (as said many times in the body of the paper), could improve the estimation performance maximizing the received \ac{SNR}, as showed in next results. As clearly visible in Fig. \ref{fig:Detection-Range-Na128}, the increase of the angle coverage costs in terms of received backscattered power (less \ac{BF} gain), and the maximum identifiability range remarkably decreases. A tradeoff appears: wider angular sectors allow to explore the environment in less time, but with limited maximum range, while narrower sectors maximize the received power and the maximum target range, at the cost of a time consuming beam sweeping search.  

In Fig. \ref{fig:Detection-Range-Na128-2Targets} the performance of the \ac{SIC} technique presented in Algorithm \ref{alg:Joint-Det-Par-Est} is showed. The scenario considers two targets, one at fixed distance of $10$ [m], the other with moving w.r.t. the x-axis, i.e., from $20$ to $150$ [m] (see Fig. \ref{fig:Ex-Scenario-MovTarget}). Note that the nearest target first interferes with the other, such that the interference term $I_p$ in Algorithm \ref{alg:Joint-Det-Par-Est} is exploited, then completely masks the far away target, such that the \ac{SIC} technique becomes necessary. As clearly visible, the performance in terms of \ac{RMSE} remains the same while considering one or two targets, as a confirmation of the validity of the proposed algorithm. The \ac{SIC} starts fail around $90$ [m], i.e., when the range difference is about $80$ [m], such that the masking effect is not removed efficiently and the far away target is not detected. Finally, the curve flats to $P_d=0.5$, because one target out of two is always correctly detected. Note that the red lines of Fig. \ref{fig:Detection-Range-Na128-2Targets} correspond to the blue ones of Fig. \ref{fig:Detection-Range-Na128}. 

Fig. \ref{fig:BF-Targets} depicts the scenario of Fig. \ref{fig:Operational-Modes} on the left side, i.e., a \ac{Tx} \ac{BF} different beams carrying their own information towards multiple targets.\footnote{Theoretically, targets positions (Doppler-delay-angle plane) are granted by some tracking algorithm which processes the radar information to produce an estimation of the (updated) targets locations. In sight of this, we suppose the target positioned within the 3-dB beamwidth of the antenna beam pattern, and the \ac{AoA} \ac{ML} search is performed within that range.} Since the presence of the target within the illuminated sector is given for granted, detection performance is not shown. In this scenario we consider three different targets within an angular sector of $10^\circ$ degrees, such that the \ac{RMSE} performance is related to the target whose range is indicated on the x-axis, while the other two targets act as interference (exploiting the use of Algorithm \ref{alg:Joint-Det-Par-Est} in all possible configurations). Observing Fig. \ref{fig:BF-Targets}, it is clear that performance depends on the number of antennas used (while $\Nrf=8$ is kept constant), since the \ac{Tx} \ac{BF} gain $G_{\mathrm{Tx}}$ is almost equal to $\Na$, i.e., $G_{\mathrm{Tx}}\simeq\Na$. Thus, a larger antenna array size reflects on better \ac{RMSE} performance, confirmed by the corresponding \ac{CRLB}, and larger maximum detectable range (greater received backscattered power). Moreover, note that a (reversed) ``waterfall'' behavior is shown for range and velocity estimation. This is because, even if the presence of the target is given for granted, low \ac{SNR} values might still lead to a large error during the Doppler-delay \ac{ML} maximization (see Algorithm \ref{alg:Joint-Det-Par-Est}). The waterfall behavior is typical of \ac{ML} estimators and has been extensively analyzed in \cite{gaudio2019effectiveness}. Also note that the \ac{AoA} \ac{RMSE} performance is upper limited by the 3-dB beamwidth of the beam pattern (see, e.g., \cite{friedlander2012transmit,visser2006array}). In fact, as the target position lies within the 3-dB beamwidth, also the \ac{AoA} estimation is limited to that range. As a consequence, the \ac{RMSE} does not exceed a systematic error, indicated as $\epsilon_\mathrm{BW}$, calculated by randomly chosen an \ac{AoA} within the range of possibilities. This behavior could be detectable also for range and velocity estimation errors, but at lower \acp{SNR} values, i.e., for much larger range.  

??? Comment on poor velocity estimation ???



==> TX_BF_90.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=7.869in,
height=4.851in,
at={(1.504in,0.803in)},
scale only axis,
xmin=-90,
xmax=90,
xlabel style={font=\color{white!25!black}},
xlabel={Angle (deg)},
ymin=-35,
ymax=0,
ylabel style={font=\color{white!25!black}},
ylabel={Radiation power (dB)},
axis background/.style={fill=white},
label style={font=\huge},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
tick style={font=\huge},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=1.0pt]
  table[row sep=crcr]{%
-90	-23.6772024059165\\
-89	-23.6773195562523\\
-88	-23.679073696774\\
-87	-23.6866114145597\\
-86	-23.7064026783307\\
-85	-23.7457641969858\\
-84	-23.8092396011055\\
-83	-23.8916950919574\\
-82	-23.968246052544\\
-81	-23.9860929174503\\
-80	-23.8734642159239\\
-79	-23.5838797795119\\
-78	-23.1608427810959\\
-77	-22.7638630513737\\
-76	-22.6367966745499\\
-75	-23.0819595427799\\
-74	-24.50891348851\\
-73	-27.5969544748774\\
-72	-32.4220057076918\\
-71	-29.6139242334133\\
-70	-24.9982054632196\\
-69	-23.0461351759451\\
-68	-23.4533026547932\\
-67	-26.0855869515697\\
-66	-26.8040614651395\\
-65	-23.2460115392072\\
-64	-21.856466967356\\
-63	-24.0106435448\\
-62	-28.3134397774129\\
-61	-23.6038547395767\\
-60	-21.6205616003307\\
-59	-25.109775300183\\
-58	-26.3252468606983\\
-57	-20.819992492392\\
-56	-22.0109280115411\\
-55	-27.6736205417359\\
-54	-20.1969032501077\\
-53	-20.9859417704977\\
-52	-27.9175834126525\\
-51	-17.4218438591522\\
-50	-19.7601096824164\\
-49	-20.48491744895\\
-48	-12.8859006812871\\
-47	-23.1447115063603\\
-46	-7.570626914828\\
-45	-1.00961063734365\\
-44	0\\
-43	-1.05907334083051\\
-42	-0.373476061241402\\
-41	-0.441148734559644\\
-40	-0.800227534268247\\
-39	-0.275053858165882\\
-38	-0.755345915158886\\
-37	-0.432649964464427\\
-36	-0.562523443217594\\
-35	-0.575218119353563\\
-34	-0.464476597122928\\
-33	-0.666651414450239\\
-32	-0.381687805144438\\
-31	-0.716881511012446\\
-30	-0.375059813762051\\
-29	-0.673312620699475\\
-28	-0.369458990646111\\
-27	-0.632835031106519\\
-26	-0.479094888267687\\
-25	-0.586961580929432\\
-24	-0.493673278427494\\
-23	-0.5923194814514\\
-22	-0.494076984024144\\
-21	-0.526455996758016\\
-20	-0.520638381496199\\
-19	-0.554488096181875\\
-18	-0.52557648646273\\
-17	-0.545268383161932\\
-16	-0.518966883560486\\
-15	-0.537053087046284\\
-14	-0.524852492652675\\
-13	-0.563983249378772\\
-12	-0.525346302828433\\
-11	-0.507864688703473\\
-10	-0.535200175875822\\
-9	-0.514996710041983\\
-8	-0.520070192860631\\
-7	-0.639058220165803\\
-6	-0.539911088097029\\
-5	-0.503736214825785\\
-4	-0.525275251618104\\
-3	-0.476055838547841\\
-2	-0.724769259870058\\
-1	-0.246703676091741\\
0	-0.747408352900553\\
1	-0.24670367609175\\
2	-0.724769259870058\\
3	-0.476055838547823\\
4	-0.525275251618119\\
5	-0.503736214825796\\
6	-0.539911088097043\\
7	-0.639058220165778\\
8	-0.520070192860676\\
9	-0.514996710041997\\
10	-0.535200175875834\\
11	-0.507864688703464\\
12	-0.525346302828465\\
13	-0.563983249378765\\
14	-0.524852492652682\\
15	-0.537053087046289\\
16	-0.518966883560491\\
17	-0.545268383161932\\
18	-0.525576486462737\\
19	-0.554488096181872\\
20	-0.520638381496199\\
21	-0.526455996758019\\
22	-0.494076984024144\\
23	-0.592319481451403\\
24	-0.493673278427494\\
25	-0.586961580929438\\
26	-0.479094888267694\\
27	-0.632835031106527\\
28	-0.369458990646097\\
29	-0.673312620699474\\
30	-0.375059813762053\\
31	-0.716881511012449\\
32	-0.381687805144441\\
33	-0.666651414450238\\
34	-0.464476597122924\\
35	-0.575218119353552\\
36	-0.562523443217595\\
37	-0.432649964464431\\
38	-0.755345915158886\\
39	-0.275053858165892\\
40	-0.800227534268247\\
41	-0.441148734559621\\
42	-0.373476061241402\\
43	-1.05907334083052\\
44	-2.89298239965987e-14\\
45	-1.00961063734365\\
46	-7.570626914828\\
47	-23.1447115063608\\
48	-12.8859006812871\\
49	-20.48491744895\\
50	-19.7601096824164\\
51	-17.4218438591521\\
52	-27.9175834126523\\
53	-20.9859417704976\\
54	-20.1969032501077\\
55	-27.6736205417358\\
56	-22.0109280115411\\
57	-20.819992492392\\
58	-26.3252468606983\\
59	-25.1097753001831\\
60	-21.6205616003307\\
61	-23.6038547395767\\
62	-28.3134397774128\\
63	-24.0106435448\\
64	-21.856466967356\\
65	-23.2460115392072\\
66	-26.8040614651396\\
67	-26.0855869515698\\
68	-23.4533026547932\\
69	-23.0461351759451\\
70	-24.9982054632195\\
71	-29.613924233413\\
72	-32.4220057076918\\
73	-27.5969544748774\\
74	-24.5089134885099\\
75	-23.0819595427799\\
76	-22.6367966745499\\
77	-22.7638630513737\\
78	-23.1608427810959\\
79	-23.5838797795119\\
80	-23.8734642159239\\
81	-23.9860929174504\\
82	-23.968246052544\\
83	-23.8916950919574\\
84	-23.8092396011055\\
85	-23.7457641969858\\
86	-23.7064026783307\\
87	-23.6866114145597\\
88	-23.679073696774\\
89	-23.6773195562523\\
90	-23.6772024059165\\
};
%\addlegendentry{data1}

\end{axis}

\begin{axis}[%
width=11.573in,
height=7.302in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> TX_BF_90_polar.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> TX_BF_90_zoom.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.701in,
height=2.111in,
at={(1.124in,0.355in)},
scale only axis,
xmin=-55,
xmax=55,
ymin=-3,
ymax=0,
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
-90	-23.6772024059165\\
-89	-23.6773195562523\\
-88	-23.679073696774\\
-87	-23.6866114145597\\
-86	-23.7064026783307\\
-85	-23.7457641969858\\
-84	-23.8092396011055\\
-83	-23.8916950919574\\
-82	-23.968246052544\\
-81	-23.9860929174503\\
-80	-23.8734642159239\\
-79	-23.5838797795119\\
-78	-23.1608427810959\\
-77	-22.7638630513737\\
-76	-22.6367966745499\\
-75	-23.0819595427799\\
-74	-24.50891348851\\
-73	-27.5969544748774\\
-72	-32.4220057076918\\
-71	-29.6139242334133\\
-70	-24.9982054632196\\
-69	-23.0461351759451\\
-68	-23.4533026547932\\
-67	-26.0855869515697\\
-66	-26.8040614651395\\
-65	-23.2460115392072\\
-64	-21.856466967356\\
-63	-24.0106435448\\
-62	-28.3134397774129\\
-61	-23.6038547395767\\
-60	-21.6205616003307\\
-59	-25.109775300183\\
-58	-26.3252468606983\\
-57	-20.819992492392\\
-56	-22.0109280115411\\
-55	-27.6736205417359\\
-54	-20.1969032501077\\
-53	-20.9859417704977\\
-52	-27.9175834126525\\
-51	-17.4218438591522\\
-50	-19.7601096824164\\
-49	-20.48491744895\\
-48	-12.8859006812871\\
-47	-23.1447115063603\\
-46	-7.570626914828\\
-45	-1.00961063734365\\
-44	0\\
-43	-1.05907334083051\\
-42	-0.373476061241402\\
-41	-0.441148734559644\\
-40	-0.800227534268247\\
-39	-0.275053858165882\\
-38	-0.755345915158886\\
-37	-0.432649964464427\\
-36	-0.562523443217594\\
-35	-0.575218119353563\\
-34	-0.464476597122928\\
-33	-0.666651414450239\\
-32	-0.381687805144438\\
-31	-0.716881511012446\\
-30	-0.375059813762051\\
-29	-0.673312620699475\\
-28	-0.369458990646111\\
-27	-0.632835031106519\\
-26	-0.479094888267687\\
-25	-0.586961580929432\\
-24	-0.493673278427494\\
-23	-0.5923194814514\\
-22	-0.494076984024144\\
-21	-0.526455996758016\\
-20	-0.520638381496199\\
-19	-0.554488096181875\\
-18	-0.52557648646273\\
-17	-0.545268383161932\\
-16	-0.518966883560486\\
-15	-0.537053087046284\\
-14	-0.524852492652675\\
-13	-0.563983249378772\\
-12	-0.525346302828433\\
-11	-0.507864688703473\\
-10	-0.535200175875822\\
-9	-0.514996710041983\\
-8	-0.520070192860631\\
-7	-0.639058220165803\\
-6	-0.539911088097029\\
-5	-0.503736214825785\\
-4	-0.525275251618104\\
-3	-0.476055838547841\\
-2	-0.724769259870058\\
-1	-0.246703676091741\\
0	-0.747408352900553\\
1	-0.24670367609175\\
2	-0.724769259870058\\
3	-0.476055838547823\\
4	-0.525275251618119\\
5	-0.503736214825796\\
6	-0.539911088097043\\
7	-0.639058220165778\\
8	-0.520070192860676\\
9	-0.514996710041997\\
10	-0.535200175875834\\
11	-0.507864688703464\\
12	-0.525346302828465\\
13	-0.563983249378765\\
14	-0.524852492652682\\
15	-0.537053087046289\\
16	-0.518966883560491\\
17	-0.545268383161932\\
18	-0.525576486462737\\
19	-0.554488096181872\\
20	-0.520638381496199\\
21	-0.526455996758019\\
22	-0.494076984024144\\
23	-0.592319481451403\\
24	-0.493673278427494\\
25	-0.586961580929438\\
26	-0.479094888267694\\
27	-0.632835031106527\\
28	-0.369458990646097\\
29	-0.673312620699474\\
30	-0.375059813762053\\
31	-0.716881511012449\\
32	-0.381687805144441\\
33	-0.666651414450238\\
34	-0.464476597122924\\
35	-0.575218119353552\\
36	-0.562523443217595\\
37	-0.432649964464431\\
38	-0.755345915158886\\
39	-0.275053858165892\\
40	-0.800227534268247\\
41	-0.441148734559621\\
42	-0.373476061241402\\
43	-1.05907334083052\\
44	-2.89298239965987e-14\\
45	-1.00961063734365\\
46	-7.570626914828\\
47	-23.1447115063608\\
48	-12.8859006812871\\
49	-20.48491744895\\
50	-19.7601096824164\\
51	-17.4218438591521\\
52	-27.9175834126523\\
53	-20.9859417704976\\
54	-20.1969032501077\\
55	-27.6736205417358\\
56	-22.0109280115411\\
57	-20.819992492392\\
58	-26.3252468606983\\
59	-25.1097753001831\\
60	-21.6205616003307\\
61	-23.6038547395767\\
62	-28.3134397774128\\
63	-24.0106435448\\
64	-21.856466967356\\
65	-23.2460115392072\\
66	-26.8040614651396\\
67	-26.0855869515698\\
68	-23.4533026547932\\
69	-23.0461351759451\\
70	-24.9982054632195\\
71	-29.613924233413\\
72	-32.4220057076918\\
73	-27.5969544748774\\
74	-24.5089134885099\\
75	-23.0819595427799\\
76	-22.6367966745499\\
77	-22.7638630513737\\
78	-23.1608427810959\\
79	-23.5838797795119\\
80	-23.8734642159239\\
81	-23.9860929174504\\
82	-23.968246052544\\
83	-23.8916950919574\\
84	-23.8092396011055\\
85	-23.7457641969858\\
86	-23.7064026783307\\
87	-23.6866114145597\\
88	-23.679073696774\\
89	-23.6773195562523\\
90	-23.6772024059165\\
};
%\addlegendentry{data1}

\end{axis}

\begin{axis}[%
width=8.646in,
height=2.667in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> peak_vs-Thr_90m_B17_F2and3.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=-50,
xmax=50,
ymin=0,
ymax=10,
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, mark=x, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-45	0.340584928356412\\
-44	0.273259165092448\\
-43	0.221043355746391\\
-42	0.23825938887424\\
-41	0.273122276605309\\
-40	0.308952993307159\\
-39	0.376861720461947\\
-38	0.402811369194718\\
-37	0.419942752756006\\
-36	0.407676530998461\\
-35	0.388069118465736\\
-34	0.429315533247556\\
-33	0.419277726471036\\
-32	0.244215413072713\\
-31	0.269146875192596\\
-30	0.29372637197988\\
-29	0.35825005345084\\
-28	0.248550983692803\\
-27	0.278721605499447\\
-26	0.312031322186295\\
-25	0.33720862267501\\
-24	0.352407588031708\\
-23	0.396958316856178\\
-22	0.334655255492181\\
-21	0.412699737677661\\
-20	0.449910629097583\\
-19	0.399078807170711\\
-18	0.402107166545867\\
-17	0.362125216767726\\
-16	0.309085602675522\\
-15	0.246461541194868\\
-14	0.188198993029135\\
-13	0.32154391620664\\
-12	0.297040884311198\\
-11	0.344910872369437\\
-10	0.467407123310925\\
-9	1.50011226834176\\
-8	4.50602399346014\\
-7	6.74738049093007\\
-6	7.30930132979663\\
-5	9.37294886315965\\
-4	9.66962152590762\\
-3	6.26852388699917\\
-2	4.4556438344855\\
-1	2.17886465207037\\
0	1.23603083073782\\
1	1.91648857228351\\
2	1.67835736470263\\
3	0.81480431104959\\
4	0.291965908265089\\
5	0.268093482346049\\
6	0.296447966618318\\
7	0.299669633416123\\
8	0.282471047003394\\
9	0.356150759632139\\
10	0.35924523157487\\
11	0.328111160033053\\
12	0.403722930237108\\
13	0.476768474200801\\
14	0.394917747363014\\
15	0.29815755498057\\
16	0.365544120714714\\
17	0.324904025892069\\
18	0.597448101491727\\
19	0.979261734985584\\
20	1.00747801432571\\
21	1.09006092030744\\
22	1.70266404334701\\
23	1.93898049650731\\
24	1.23457871234937\\
25	0.759624482087902\\
26	0.491481530357319\\
27	0.286765180474164\\
28	0.309125284848845\\
29	0.271329986331834\\
30	0.246118154436242\\
31	0.31304053996812\\
32	0.322009468812547\\
33	0.259269359794272\\
34	0.289621526792322\\
35	0.33483793186421\\
36	0.309806514834611\\
37	0.279017339569036\\
38	0.329444535362534\\
39	0.398456846305047\\
40	0.375408472462723\\
41	0.38505867325091\\
42	0.407233003070955\\
43	0.573631939323292\\
44	0.542546446746401\\
45	0.439809035726439\\
};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
-45	0.409683414907964\\
-44	0.409888747638672\\
-43	0.463429489960739\\
-42	0.510877392534618\\
-41	0.565292580692921\\
-40	0.582103677698604\\
-39	0.604217053792077\\
-38	0.604217053792077\\
-37	0.604217053792077\\
-36	0.604217053792077\\
-35	0.604217053792077\\
-34	0.604217053792077\\
-33	0.604217053792077\\
-32	0.582103677698604\\
-31	0.53737508017626\\
-30	0.528611382047562\\
-29	0.528611382047562\\
-28	0.505812934012515\\
-27	0.505812934012515\\
-26	0.528611382047562\\
-25	0.53737508017626\\
-24	0.595437475284267\\
-23	0.595437475284267\\
-22	0.595437475284267\\
-21	0.595437475284267\\
-20	0.595437475284267\\
-19	0.595437475284267\\
-18	0.595437475284267\\
-17	0.543187825151588\\
-16	0.598618210756067\\
-15	0.598618210756067\\
-14	0.598618210756067\\
-13	0.6031607498188\\
-12	0.701110684966387\\
-11	2.25016840251264\\
-10	6.7590359901902\\
-9	9.40278583049875\\
-8	9.40278583049875\\
-7	9.40278583049875\\
-6	9.40278583049875\\
-5	9.40278583049875\\
-4	9.40278583049875\\
-3	9.40278583049875\\
-2	9.40278583049875\\
-1	6.68346575172825\\
0	3.26829697810555\\
1	2.87473285842527\\
2	2.51753604705395\\
3	1.85404624610673\\
4	1.22220646657439\\
5	0.538867847362305\\
6	0.538867847362305\\
7	0.538867847362305\\
8	0.538867847362305\\
9	0.534226139448208\\
10	0.538867847362305\\
11	0.538867847362305\\
12	0.548316181072071\\
13	0.592376621044521\\
14	0.605584395355662\\
15	0.715152711301201\\
16	0.896172152237591\\
17	1.46889260247838\\
18	1.51121702148857\\
19	1.51121702148857\\
20	1.51121702148857\\
21	1.51121702148857\\
22	1.51121702148857\\
23	1.51121702148857\\
24	1.51121702148857\\
25	1.51121702148857\\
26	1.13943672313185\\
27	0.737222295535979\\
28	0.483014203218821\\
29	0.483014203218821\\
30	0.469560809952179\\
31	0.464709772251916\\
32	0.464709772251916\\
33	0.469560809952179\\
34	0.483014203218821\\
35	0.494166803043801\\
36	0.502256897796315\\
37	0.563112708694085\\
38	0.577588009876364\\
39	0.59768526945757\\
40	0.59768526945757\\
41	0.59768526945757\\
42	0.59768526945757\\
43	0.59768526945757\\
44	0.59768526945757\\
45	0.577588009876364\\
};
\addlegendentry{data2}


%%%%%% 3Fingers
\addplot [color=mycolor1, mark=x, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-45	0.798773790723651\\
-44	0.651996015565162\\
-43	0.845960936579404\\
-42	0.818556092210552\\
-41	0.787805174737237\\
-40	0.956566526353864\\
-39	0.932432552485206\\
-38	0.998115004292475\\
-37	1.00171275622019\\
-36	0.848398580501932\\
-35	0.981623762551846\\
-34	1.02412779811732\\
-33	0.817717077155478\\
-32	0.920763486451311\\
-31	0.921050095685397\\
-30	0.877693904232812\\
-29	0.991864744065287\\
-28	1.0298143738001\\
-27	0.792727501356741\\
-26	0.711825902126444\\
-25	0.747009549180511\\
-24	1.30015138618535\\
-23	1.40119368585642\\
-22	1.25502271788672\\
-21	1.08565593153814\\
-20	1.04642511680175\\
-19	1.00204832937917\\
-18	0.935883249995972\\
-17	0.920820633995211\\
-16	1.09895128230448\\
-15	0.920449652717067\\
-14	0.759133712817625\\
-13	0.75157409068371\\
-12	0.767798142248308\\
-11	0.684356610305236\\
-10	0.96055686586232\\
-9	1.02166815848765\\
-8	0.865073565821297\\
-7	0.847105742373743\\
-6	1.68186737390521\\
-5	2.25022765256608\\
-4	2.62125499208181\\
-3	2.21756675201337\\
-2	1.06896790095634\\
-1	0.857938017659404\\
0	0.834144443236197\\
1	0.835627480219192\\
2	0.841937514123164\\
3	0.676714513818195\\
4	0.555391311456488\\
5	0.526514364812319\\
6	1.0106551616413\\
7	1.03962461932378\\
8	1.35703628970855\\
9	1.07536747429293\\
10	0.755065898277111\\
11	0.972904161164631\\
12	0.905498844796574\\
13	1.16996977329018\\
14	0.917072753184917\\
15	0.656754299105802\\
16	0.765726555444321\\
17	0.733356545829057\\
18	0.743131702422227\\
19	1.01766618794126\\
20	0.894502003471086\\
21	0.648594974144041\\
22	1.09398591434788\\
23	0.892006964860444\\
24	0.464574375804009\\
25	0.612705803696415\\
26	0.690713500167987\\
27	1.13070383210223\\
28	1.38480828022908\\
29	0.901660128436403\\
30	0.877834336293914\\
31	0.89644098894774\\
32	0.763675212535792\\
33	0.823445854967183\\
34	0.934397603678175\\
35	1.09993561106879\\
36	1.2259489679033\\
37	1.36517213333456\\
38	1.63052969357107\\
39	1.46856277558617\\
40	1.07311586694124\\
41	1.21821300149585\\
42	1.05253880021441\\
43	1.19828212085493\\
44	1.30206245337465\\
45	1.18720171904917\\
};
\addlegendentry{data1}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
-45	1.19816068608548\\
-44	1.22783413831583\\
-43	1.26894140486911\\
-42	1.2725978707529\\
-41	1.39864882872781\\
-40	1.4348497895308\\
-39	1.4348497895308\\
-38	1.4348497895308\\
-37	1.4348497895308\\
-36	1.4348497895308\\
-35	1.47243564382777\\
-34	1.48779711609793\\
-33	1.48779711609793\\
-32	1.47243564382777\\
-31	1.3815751435281\\
-30	1.47243564382777\\
-29	1.48779711609793\\
-28	1.48779711609793\\
-27	1.54472156070015\\
-26	1.56963767520263\\
-25	1.56963767520263\\
-24	1.56963767520263\\
-23	1.56963767520263\\
-22	1.62848389730721\\
-21	1.62848389730721\\
-20	1.62848389730721\\
-19	1.62848389730721\\
-18	1.56963767520263\\
-17	1.50307249406876\\
-16	1.44083529879348\\
-15	1.44083529879348\\
-14	1.40382487499396\\
-13	1.38123095099282\\
-12	1.38123095099282\\
-11	1.44083529879348\\
-10	1.44083529879348\\
-9	1.53250223773148\\
-8	1.60345185143452\\
-7	1.60345185143452\\
-6	1.60345185143452\\
-5	1.60345185143452\\
-4	1.60345185143452\\
-3	1.60345185143452\\
-2	1.60345185143452\\
-1	1.60345185143452\\
0	1.51598274246196\\
1	1.51598274246196\\
2	1.51598274246196\\
3	1.51598274246196\\
4	1.28690702648911\\
5	1.45935624174695\\
6	1.45935624174695\\
7	1.51598274246196\\
8	1.51598274246196\\
9	1.51598274246196\\
10	1.51598274246196\\
11	1.51598274246196\\
12	1.45935624174695\\
13	1.45935624174695\\
14	1.37560912977738\\
15	1.35824826719486\\
16	1.37560912977738\\
17	1.35824826719486\\
18	1.34175300520663\\
19	1.33801044729067\\
20	1.14858983316648\\
21	1.33801044729067\\
22	1.34175300520663\\
23	1.3524901926546\\
24	1.3524901926546\\
25	1.34466148342161\\
26	1.34466148342161\\
27	1.34466148342161\\
28	1.34466148342161\\
29	1.3524901926546\\
30	1.40159640551726\\
31	1.64990341660318\\
32	1.69605574815334\\
33	1.83892345185495\\
34	1.64990341660318\\
35	1.82731950224377\\
36	1.82731950224377\\
37	1.82731950224377\\
38	1.83892345185495\\
39	1.83892345185495\\
40	1.83892345185495\\
41	1.83892345185495\\
42	1.82731950224377\\
43	1.7974231812824\\
44	1.78080257857375\\
45	1.60967380041186\\
};
\addlegendentry{data2}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
